A Review of Differentiable Simulators

Differentiable simulators continue to push the state of the art across a range of domains including computational physics, robotics, and machine learning. Their main value is the ability to compute gradients of physical processes, which allows differentiable simulators to be readily integrated into commonly employed gradient-based optimization schemes. To achieve this, a number of design decisions need to be considered representing trade-offs in versatility, computational speed, and accuracy of the gradients obtained. This paper presents an in-depth review of the evolving landscape of differentiable physics simulators. We introduce the foundations and core components of differentiable simulators alongside common design choices. This is followed by a practical guide and overview of open-source differentiable simulators that have been used across past research. Finally, we review and contextualize prominent applications of differentiable simulation. By offering a comprehensive review of the current state-of-the-art in differentiable simulation, this work aims to serve as a resource for researchers and practitioners looking to understand and integrate differentiable physics within their research. We conclude by highlighting current limitations as well as providing insights into future directions for the field.

==> Images/growth.tex <==
\pgfplotstableread[col sep=comma]{Images/growth.csv}\data
\begin{figure}
    \centering
\begin{tikzpicture}    
    \begin{axis}[
        name=mainplot,
        xmin = 2010, xmax = 2023,
        ymin = 0, ymax = 60,
        enlarge y limits=true,
        width = 0.5\textwidth,
        % grid=major,
        ymajorgrids,
        height = 0.28\textwidth,                
        xtick=data,
        xtick style={draw=none},
        xticklabel style={/pgf/number format/1000 sep=,rotate=60,anchor=east,font=\scriptsize},
        ylabel= \# Papers,
        ]
        
        \addplot[red, mark=none] table[x=y , y=n] {\data};
        \addplot[mark=none, draw=none, name path=A] coordinates {(2016,-200) (2016,200)};
        \addplot[mark=none, draw=none, name path=B] coordinates {(2023,-200) (2023,200)};
        \addplot+[green, fill opacity=0.2] fill between[of=A and B,soft clip={domain=1990:2030}];
        \node[scale=0.9] at (axis cs: 2020.5,60) {{\normalsize Span Of Our Review}};
        \end{axis}
\end{tikzpicture}
    \caption{Growth}
    \label{fig:enter-label}
\end{figure}


==> Sections/11_Optimisatation.tex <==
\subsection{Optimization Methods}
% Rhys

% Algorithms:
% First order methods:
%   - Gradient descent
%   - Stochastic gradient descent
%   - ADAM
%   - MDMM (for constrained optimization, seems a lot like the Arrow-Hurwitz method tbh)
% Quasi-Newton methods:
%   - L-BFGS
%   - L-BFGS-B
%   - SQP w/ BFGS updates

% Trajectory optimization modeling:
%   - NLopt (SQP using BFGS)

% Applications which utilize differentiable simulators all fundamentally involve solving an optimization problem. Therefore, optimization algorithms are at the core of utilizing gradients from differentiable simulators to efficiently perform a task.

As all applications involve solving an optimization problem, algorithms which can minimize or maximize an objective are at the core of utilizing gradients from differentiable simulators to efficiently perform a task. A list of common optimization algorithms used with differentiable simulators is summarized in~\cref{tab:opt}.

First-order methods are optimization algorithms which only require oracles providing the function value and gradient of the objective being minimized. These are widely employed in differentiable simulation for their simplicity and capacity to handle large problem dimensions. The basic approach, exemplified by gradient descent, involves taking steps in the direction of the negative gradient at each iteration, i.e., at the $k$-th iteration
\begin{equation}
    \theta_{k+1} = \theta_k - t_k \frac{d\mathcal{L}}{d\theta},
\end{equation}
where $\mathcal{L}:\mathbb{R}^p\rightarrow\mathbb{R}$ is the objective function, $\theta\in\mathbb{R}^p$ is the vector of $p$ parameters being optimized over, and $t_k>0$ is a step size. Gradient descent, in addition to common variations of the algorithm used in deep learning such as ADAM~\cite{kingma-2014-adam-optimization}, RMSProp~\cite{hinton-2012-neural-descent}, and stochastic gradient descent~\cite{saad-1998-online-approximations}, are the most popular optimization techniques in applications of differentiable simulators.
% First-order methods are the most common class of methods used in differentiable simulation due to their simplicity and ability to scale to large problem dimensions. Gradient descent based methods are the most popular technique for optimization, this includes gradient descent, as well as variations of gradient-descent like ADAM~\cite{kingma-2014-adam-optimization}, RMSProp\cite{hinton-2012-neural-descent}, SGD~\cite{saad-1998-online-approximations} commonly used in deep learning application. These methods are almost used interchangabely with them being very easily changed between in modern deep learning frameworks. To handle constraints, the Modified Differential Multiplier Method~\citep{platt-1987-constrained-optimziation} has been applied in grasping tasks~\citep{turpin-2022-grasp-hands}.
% Gradient descent methods have been used in~\citep{de-2018-end-control, hu-2019-chainqueen-robotics, qiao-2020-scalable-control, jatavallabhula-2021-gradsim-control, sundaresan-2022-diffcloud-objects, zhong-2021-extending-models, wang-2022-real2sim2real-engine, wang-2023-softzoo-environments}. For problems optimizing over large sets of data, stochastic gradient descent~\citep{saad-1998-online-approximations} has been employed with good performance~\citep{liang-2019-differentiable-problems}. The Adam optimizer~\citep{kingma-2014-adam-optimization}, which augments gradient descent with a momentum term, has gained popularity for both optimization~\citep{huang-2021-plasticinelab-physics, turpin-2022-grasp-hands, zhong-2021-extending-models, le-2023-differentiable-objects, arnavaz-2023-differentiable-simulations, chen-2022-imitation-physics} and training models with a differentiable simulation based loss~\citep{scibior-2021-imagining-simulation}. 
% L-BFGS-B, an extension of L-BFGS, has also been employed in scenarios~\citep{li-2022-diffcloth-contact,granados-2022-model-physics,Xu-2021-An-Design}. For morphology optimization, SLSQP (Sequential Least Squares Quadratic Programming) method \citep{kraft-1988-a-programming} has been used commonly~\citep{hu-2019-chainqueen-robotics,zhao-2022-graph-robots,zhao-2022-automatic-grammar}. Trust Region methods \citep{byrd-1987-trust-optimization} have been employed for differentiable musculotendon modeling~\citep{wang-2022-differentiable-musculotendons}. 


\begin{table}[tb!]
\centering
\begin{tabular}{|l|l|}
\hline
Method & Frequency \\ \hline
Gradient Descent & 9 \\
ADAM & 28 \\
Stochastic Gradient Descent (SGD) & 9 \\
RMSProp & 1 \\
(Limited memory) BFGS & 8 \\
Sequential Least Squares QP& 3 \\
\hline
\end{tabular}
\caption{Popularity of common optimization methods. Numbers represent the frequency of use.}
\label{tab:opt}
\end{table}






% Add second order paper


% alpha-order: suh-2022-do-gradients
% Smoothed gradients: zhu-2023-difflfd-rendering, suh-2022-do-gradients

% Second order: mora-2021-pods-simulation

Another class of optimization algorithms are second-order methods, which use Hessian oracles to find improved step directions. This allows the optimization algorithm to converge in significantly fewer iterations. However the Hessian of the objective needs to be inverted at every iteration, which can be prohibitively expensive at large problem dimensions. \citet{zimmermann2019optimal} extend the adjoint method (see Section~\ref{subsubsec:analytical}) to obtain the Hessian of an objective function analytically at a relatively low cost. This method is applied in~\cite{mora-2021-pods-simulation}, where the Hessian is used to implement a second-order Newton method for policy optimization. Characteristic of second-order methods, the authors show that the second-order updates converge significantly faster than a simple gradient descent update. Other works have employed quasi-Newton methods, which approximate second-order methods without having to explicitly form the inverse Hessian of the objective, and like first-order methods only require function value and gradient oracles. One widely utilized optimization algorithm is the limited-memory Broyden-Fletcher-Goldfarb-Shanno (L-BFGS) method~\citep{liu-1989-on-optimization}, which has been used in many applications ranging between system identification, trajectory optimization, and morphology optimization~\citep{heiden-2019-interactive-simulation,li-2023-learning-simulation,du-2021-diffpd-dynamics,geilinger-2020-add-contact}. 


In~\cite{suh-2022-do-gradients}, concerns are raised about the usefulness or accuracy of gradients obtained from differentiable simulators, particularly around discontinuities like those from contact models. To address this, a ``zeroth-order'' gradient estimate, obtained by sampling the function value, is proposed to mitigate these issues. An ``$\alpha$-order'' gradient is then introduced by interpolating between first-order and zeroth-order gradients. A similar approach is adopted by~\cite{lelidec-2022-augmenting-smoothing,zhu-2023-difflfd-rendering}, which uses an averaged gradient over a probabilistic distribution at a point. Similar observations were made in~\cite{werling-2021-fast-contact}, which shows how a heuristic perturbation of the true gradients of the simulator can help optimizers avoid getting stuck in saddle-points. 




% Constrained optimization: turpin-2022-grasp-hands
% - L-BFGS-B is variant of L-BFGS that supports box-constraints. Using an active-set method. \citep{li-2022-diffcloth-contact,granados-2022-model-physics,Xu-2021-An-Design}

% - Trust region Levenberg Marquardt algorithm with bounds, by the Ceres solver. Augments with a projected line search in the direction of the trust region LM \cite{collins-2021-follow-realitygrad}

% - SLSQP, from NLOpt, solves problem by approximating the problem as a sequence of (possibly constrained) least squares subproblems, for which there are well-known methods of solving. \citep{hu-2019-chainqueen-robotics,zhao-2022-graph-robots,zhao-2022-automatic-grammar}

% - the Modified Differential Multiplier Method~\citep{platt-1987-constrained-optimziation} has been applied in grasping tasks~\citep{turpin-2022-grasp-hands}. Type of first-order primal-dual algorithm.

Often, optimization problems involve constraints on the decision variables. One simple type of constraint is box constraints, i.e.
\begin{equation}
    \theta_{\textnormal{min}} \leq \theta \leq \theta_{\textnormal{max}},
\end{equation}
where $\theta_{min},\theta_{max}\in\mathbb{R}^p$ are the minimum and maximum allowable values of the parameters. For these problems, projected gradient descent can be employed (see, e.g.,~\cite{beck2017first}), which clamps each variable within specified bounds after each gradient descent step. Alternatively, in~\citep{li-2022-diffcloth-contact,granados-2022-model-physics,Xu-2021-An-Design}, an active-set variant of L-BFGS which supports box constraints, called L-BFGS-B, is used to solve constrained optimization problems. In \citet{collins-2021-follow-realitygrad}, a trust region Levenberg Marquardt algorithm from the Ceres solver~\citep{Agarwal_Ceres_Solver_2022} is used, supporting box constraints through a projected line search. Handling more complex constraints, such as those in trajectory optimization, \citep{hu-2019-chainqueen-robotics,zhao-2022-graph-robots,zhao-2022-automatic-grammar} use the Sequential Least Squares Quadratic Programming (SLSQP) method~\citep{kraft-1988-a-programming} implemented by NLopt~\cite{NLopt}. This approximates the optimization problem as a sequence of constrained least squares subproblems, solvable using well-known methods~\citep{lawson1995solving}. In~\citep{turpin-2022-grasp-hands,Heiden2022InferringVideo}, the Modified Differential Multiplier Method~\citep{platt-1987-constrained-optimziation} is employed, handling constraints through a first-order primal-dual method, i.e., a gradient method is used to perform gradient descent on the primal variables and gradient ascent on the dual variables.


% Custom: antonova-2023-rethinking-perspective

Considering the nonconvex nature of many problems, global optimization strategies become crucial. Stochastic gradient descent and related methods, such as ADAM and momentum-based algorithms, are well-known to escape from shallow local minima (see, e.g.,~\cite{kleinberg2018alternative}). In~\cite{antonova-2023-rethinking-perspective}, a variant of Bayesian optimization tailored for rugged landscapes is employed, aiming to explore the global loss landscape while also locally optimizing regions with low loss. Similarly, \citet{gartner-2022-differentiable-reconstruction} utilizes basin-hopping, combining a local search (e.g., gradient descent) with random perturbations to escape local minima.

==> Sections/9_SoftRob.tex <==
% \subsection{Soft Robotics}




==> Sections/collage.tex <==
\begin{figure*}[htbp]
    \centering
    \setlength{\tabcolsep}{0pt} % No space between columns

    \settoheight{\maxheight}{\includegraphics{Images/collage/throw.png}}


    \begin{tabular}{@{}p{0.37\textwidth}p{0.38\textwidth}p{0.25\textwidth}@{}}
        \multirow{2}{0.37\textwidth}{\includegraphics[width=\linewidth, height=0.18\maxheight, valign=t]{Images/collage/throw.png}} &
        \multirow{2}{0.38\textwidth}{\includegraphics[width=\linewidth, height=0.18\maxheight, valign=t]{Images/collage/chop.png}} &
        \includegraphics[width=\linewidth, height=0.09\maxheight, valign=t, trim=0 0 0 4cm, clip]{Images/collage/chop2.png} \\        
        & & \includegraphics[width=\linewidth, height=0.09\maxheight, valign=t, trim=0 0 0 4cm, clip]{Images/collage/chop3.png} \\
    \end{tabular}
    \begin{tabular}{@{}p{0.25\textwidth}p{0.25\textwidth}p{0.25\textwidth}p{0.25\textwidth}@{}}
        \includegraphics[width=\linewidth, height=0.13\maxheight, valign=t, trim=32cm 0.38cm 3.5cm 16cm, clip]{Images/collage/morph2.jpg} &         \includegraphics[width=\linewidth, height=0.13\maxheight, valign=t, trim=1cm 27cm 57cm 4cm, clip]{Images/collage/morph1.jpg} &         \includegraphics[width=\linewidth, height=0.13\maxheight, valign=t, trim=26cm 27cm 32cm 4cm, clip]{Images/collage/morph1.jpg} &         \includegraphics[width=\linewidth, height=0.13\maxheight, valign=t, trim=0cm 0cm 0cm 0cm, clip]{Images/collage/deform.png}
    \end{tabular}
    \caption{Differentiable simulation applied to various tasks including (a) optimizing a throwing motion \cite{geilinger-2020-add-contact}, (b) optimizing cutting policy \cite{heiden-2021-disect-cutting}, (c) using cage-based parametrization for co-design of robotic gripper \cite{Xu-2021-An-Design} and (d) optimizing manipulation policy of deformable object \cite{li-2023-dexdeform-physics}.}
\end{figure*}


==> Sections/more_papers.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ADDITIONAL PAPERS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Follow the Gradient (RealityGrad) \cite{collins-2021-follow-realitygrad} (Jack)

Diff-LfD \cite{zhu-2023-difflfd-rendering} leverages diffsim and diff rendering for in-hand manipulation, proposes model-based LfD framework from RGB videos with unknown camera frame. Leveraging diff rendering for pose estimation and mesh reconstruction. Gradients from diffsim are used in contact-point localization and contact-wrench optimization at each time step. Results: more robust shape reconstruction and pose estimation; policies optimized using proposed framework results in more stable contacts and lower goal error rates than baselines (RRT, contact-implicit traj opt, pre-grasp informed dext manip, iLQR). 

Imitation Learning as State Matching \cite{chen-2022-imitation-physics} evaluates proposed approach on several BRAX continuous control tasks, only requiring a single expert demonstration. Leveraging differentiable dynamics to 1) avoid a typical double-loop structure of alternating between learning rewards and learning policies, and 2) gradient from the dynamics provides richer information than single reward value, guides local improvement of actions and results in less training variance. Also designed robot cloth manipulation task to demonstrate generalizability in complex tasks. Overall, ILD outperforms SOTA on 6/8 tasks, generally able to recover expert behavior, performance gain of ILD increases with more complex tasks. 

SAGCI-System \cite{lv-2022-sagci-learning} Hybrid Sim included. Policy Opt?

Variational Reparametrized Policy Learning \cite{huang-2022-variational-physics}
- learns a decoder that "reparametrizes" the random (simple) distribution z into a multi-modality distribution over entire trajectory space (instead of over action space). Learn to model the joint distribution p(z, t), where t is the sampled trajectory.
- The policy can be viewed as encoding the stochastic latent variable z into the trajectory distribution. 
- The evident lower bound (ELBO) treated as reward function
- Path-wise gradient information (trajectory w.r.t policy parameters) obtained from diffsim. Uses this first-order gradient to optimize policy parameters directly. 


==> Tables/applications_temp.tex <==

Solver-in-the-Loop: Learning from Differentiable Physics to Interact with Iterative PDE-Solvers\cite{um-2020-solver-solvers}
ADD: Analytically Differentiable Dynamics for Multi-Body Systems with Frictional Contact\cite{geilinger-2020-add-contact}
Underwater Soft Robot Modeling and Control With Differentiable Simulation\cite{du-2021-underwater-simulation}
Differentiable Physics Models for Real-world Offline Model-based Reinforcement Learning\cite{lutter-2021-differentiable-learning}
Do Differentiable Simulators Give Better Policy Gradients?\cite{suh-2022-do-gradients}
Learning to Slide Unknown Objects with Differentiable Physics Simulations\cite{song-2020-learning-simulations}
PODS: Policy Optimization via Differentiable Simulation\cite{mora-2021-pods-simulation}
DiffSkill: Skill Abstraction from Differentiable Physics for Deformable Object Manipulations with Tools\cite{lin-2022-diffskill-tools}
Imagining The Road Ahead: Multi-Agent Trajectory Prediction via Differentiable Simulation\cite{scibior-2021-imagining-simulation}
DiffCloud: Real-to-Sim from Point Clouds with Differentiable Simulation and Rendering of Deformable Objects\cite{le-2023-differentiable-objects}
Grasp'D: Differentiable Contact-rich Grasp Synthesis for Multi-fingered Hands\cite{turpin-2022-grasp-hands}
Sim2Sim Evaluation of a Novel Data-Efficient Differentiable Physics Engine for Tensegrity Robots~\cite{wang-2021-sim2sim-robots}
Real2Sim Transfer using Differentiable Physics~\cite{heiden-2019-real2sim-physics}
Rethinking Optimization with Differentiable Simulation from a Global Perspective~\cite{antonova-2023-rethinking-perspective}
Differentiable Dynamics for Articulated 3d Human Motion Reconstruction~\cite{gartner-2022-differentiable-reconstruction}
Differentiable Physics Simulation of Dynamics-Augmented Neural Objects~\cite{le-2023-differentiable-objects}
Augmenting differentiable physics with randomized smoothing~\cite{lelidec-2022-augmenting-smoothing}
Dojo: A Differentiable Physics Engine for Robotics\cite{howelll-2022-dojo-robotics}
A Recurrent Differentiable Engine for Modeling Tensegrity Robots Trainable with Low-Frequency Data\cite{wang-2022-recurrent-data}
Fast Aquatic Swimmer Optimization with Differentiable Projective Dynamics and Neural Network Hydrodynamic Models\cite{nava-2022-fast-models}
DiffSRL: Learning Dynamical State Representation for Deformable Object Manipulation With Differentiable Simulation\cite{chen-2022-diffsrl-simulation}
Model Identification and Control of a Low-cost Mobile Robot with Omnidirectional Wheels using Differentiable Physics\cite{granados-2022-model-physics}
Physical Simulation Layer for Accurate 3D Modeling~\cite{mezghanni-2022-physical-modeling}
Training Efficient Controllers via Analytic Policy Gradient~\cite{wiedemann-2023-training-gradient}
Real2Sim2Real Transfer for Control of Cable-driven Robots via a Differentiable Physics Engine\cite{wang-2022-real2sim2real-engine}
SAM-RL: Sensing-Aware Model-Based Reinforcement Learning via Differentiable Physics-Based Simulation and Rendering~\cite{lv-2022-samrl-rendering}
Real-Time Model Predictive Control and System Identification Using Differentiable Simulation~\cite{chen-2022-real-simulation}
Sim-to-Real for Soft Robots Using Differentiable FEM: Recipes for Meshing, Damping, and Actuation~\cite{dubied-2022-simtoreal-actuation}
Graph Grammar-Based Automatic Design for Heterogeneous Fleets of Underwater Robots~\cite{zhao-2022-graph-robots}
DexDeform: Dexterous Deformable Object Manipulation with Human Demonstrations and Differentiable Physics~\cite{li-2023-dexdeform-physics}
Learning Object Manipulation Skills from Video via Approximate Differentiable Physics~\cite{petrik-2022-learning-physics}
DiffMimic: Efficient Motion Mimicking with Differentiable Physics *
Improving Gradient Computation for Differentiable Physics Simulation with Contacts~\cite{zhong-2023-improving-contacts}
Differentiable Depth for Real2Sim Calibration of Soft Body Simulations~\cite{arnavaz-2023-differentiable-simulations}
Predicting Physical Object Properties from Video~\cite{link-2022-predicting-video}
Automatic Co-Design of Aerial Robots Using a Graph Grammar~\cite{zhao-2022-automatic-grammar}
Learning Tool Morphology for Contact-Rich Manipulation Tasks with Differentiable Simulation~\cite{li-2023-learning-simulation}
Follow the Gradient: Crossing the Reality Gap using Differentiable Physics (RealityGrad)~\cite{collins-2021-follow-realitygrad}
Diff-LfD: Contact-aware Model-based Learning from Visual Demonstration for Robotic Manipulation via Differentiable Physics-based Simulation and Rendering~\cite{zhu-2023-difflfd-rendering}
Imitation Learning as State Matching via Differentiable Physics~\cite{chen-2022-imitation-physics}
SAGCI-System: Towards Sample-Efficient, Generalizable, Compositional,
and Incremental Robot Learning *~\cite{lv-2022-sagci-learning}

==> notes.tex <==
draft in the next month
 - things left
    2 weeks/	
    - intro (jack)
	- background (needs full writing from dot points) (rhys, kerry)
    - brainstorm future work/discussion (each bring at least 2 points)
	- add other papers (michael)
    - big image (michael)
    
    - 2 weeks/ 
	- engine information
    - discussion/future work

other notes
- add info about adjoint method
- effecient diff sim of articulated bodies uses adjoint
- check non linear lcp

Discussion 
- Keywords
- Use of differential or differentiable
- Simulator vs. physics engine
- The use of "we" - shouldn't be used in a review

==> rebuttal.tex <==
% format like this
Reviewer#1, Concern # 1 (please list here):
Author response:
Author action: We updated the manuscript by ….

Comments:
!. More recent refs must be cited.
% expliclatally say the cut-off date. <- jack
% The reviewer is correct in pointing out that the review lacks the most recent references from 2024. To keep the review concise and complete we needed to delineate what was in and out of scope. We have more clearly delineated in text that the scope of covered literature ends without covering differentiable simulator papers from 2024.
% In the 4th paragraph of the Introduction (Section I) we have added the sentence: "To ensure comprehensive coverage, this review encompasses all relevant literature published before 2024 that proposes or utilizes differentiable physics simulators, with some necessary caveats outlined."

2. The refs must be in chronological order of the reported research and cited in the same way in paper.
Author Response: We interpret this comment, as that the references must appear in numeric order, to ensure that the first reference is [1] and so forth.
Author Action: We have update the manuscript to ensure they are in the correct order.

% reorder latex figure thing. <- rhys
% our interpataion of this is that numerical, not chronologically. review is based on group and context to help understanding
3. Authors contribution need to highlight.
% We have taken the reviewers comment on-board and added to the introduction a section that clearly defines the contributions of the paper. 
% In the 4th paragraph of the Introduction (Section I) we have added the sentence: "In summary, the contributions of this paper are, (i) a thorough review of the fundamental concepts and methodologies of differentiable physics simulators, (ii) a curated list of well-maintained differentiable simulators to aid practitioners in selecting appropriate tools, (iii) applications of differentiable simulators demonstrating how these simulators have been used in the past, and (iii) a discussion on future directions of the field."

4. Critical check for language and grammar are must.
% We have addressed the comment by the reviewer by having several native english speakers critique the review for language and grammar.
% Numerous small changes throughout the document have been made to address this.

Reviewer 2

General Feedback: Your manuscript provides a thorough and well-structured review of differentiable simulators. The breadth and depth of the coverage are impressive, and it serves as a significant contribution to the field. The systematic approach to reviewing the literature and the detailed discussion of various technical aspects of differentiable simulators are particularly commendable.
% thanks

Suggestions for Enhancement:
Practical Challenges: While the technical details are well-covered, the manuscript could benefit from a more detailed exploration of the practical challenges associated with implementing and using differentiable simulators in real-world applications. This could include discussions on computational demands, scalability, and integration with existing systems.

Author Response: Thank you for this suggestions, we have tried to add further detail about some of the practical challenges for real-world applications.

We have added discussion around this in the last paragraph of the future work section. 

% add scalability to future directions?
% parallel sim? more explicit dicsussion helps faster
% pytorch vs jax speed
% amount of time you can simulate through depends on the loss
% computational demands are depending on what you are trying to simulate, one advantage is parallelism of gpu's
% implications of scalabiltiy/demands
% highlight the parallel in each section
% integration in to workflows.
% -> rhys

Case Studies or Examples: To enhance the manuscript's applicability and readability, consider including case studies or specific examples where differentiable simulators have been successfully implemented. This could help illustrate the potential impacts and practical considerations of the technology in a more concrete manner.

Thank you for this comment and we agree that having specific examples of differentiable simulation used is very important for this survey, we believe Section IV (Application) aims to address this in a concrete manner.

% rebutt the first part, we have an applications section which aims to do this. -> rhys

Future Directions: The section on future directions is insightful but could be expanded to include emerging trends and potential interdisciplinary applications that could influence the development of differentiable simulators.

We agree that having these points are important in the future directions, however, we believe in the current manuscript the future direction already aims to discuss emerging trends and potential interdisciplinary applications. 

% rebutt -> we have this already. -> rhys

Technical Clarifications:

Gradient Calculation Methods: The section on gradient calculation is crucial; however, it might be beneficial to provide more explicit comparisons between the different methods. Clarifying the advantages, limitations, and suitable contexts for each method could aid readers in understanding why and when to choose one method over another.
% higlight limitations (pros/cons) further? hard to solve.
% be more explicit on reverse/forward, using [68] (maching learning survey) as evidence
% compare three methods in intro more explicatally.
% -> kerry

Thank you for your feedback. We had some discussion in each subsection discussing the pros and cons of each gradient calculation method. However, we have now moved this discussion up to the beginning of Section II.A: Gradient Calculation to provide a high-level, unified comparison of each method, as suggested.

Integration Methods: A more detailed discussion on the choice of integration methods, especially in the context of their stability and accuracy, would be valuable. This could be supported by comparative data or references to studies that have analyzed the performance of these methods in different settings.
% https://ieeexplore.ieee.org/abstract/document/934683 <- cloth simulation integration
% be more explicit in the intro -> kerry

We previously had some discussion about the advantages and disadvantages of explicit and implicit integration techniques. However, to improve the clarity of the paper we have moved this discussion to the beginning of Section II.D: Integrator. Here, we have added experimental results from~\cite{du-2021-diffpd-dynamics} which demonstrates the advantages of implicit integration over explicit integration, as well as~\cite{volino2001comparing} which presents further experimental results comparing between various integration schemes.



Visual and Organizational Improvements:

Figures and Tables: Consider adding more visual elements such as charts, graphs, or flow diagrams to summarize complex concepts or to compare the features and capabilities of various differentiable simulators. This would make the manuscript more engaging and accessible to readers.
% add another figure? what/where?
% diagram of sort-of-system id/loss/how the simulator works in general.
% come back to it
% add more examples of figures for applications
% -> everyone

Subsections and Headings: Some sections are dense with information. Breaking these down further into subsections or including more descriptive headings could improve readability and navigation through the document.
% breakdown applications further.
% -> everyone

Reference Check: Ensure that all references are up-to-date and include the most recent significant works in the field to maintain the manuscript’s relevance and comprehensiveness.
% add cut-off date to text
% do another de-arxiv check
% -> michael

